Learning Disentangled Prompts for Compositional Image Synthesis

We study domain-adaptive image synthesis, the problem of teaching pretrained image generative models a new style or concept from as few as one image to synthesize novel images, to better understand the compositional image synthesis. We present a framework that leverages a pretrained class-conditional generation model and visual prompt tuning. Specifically, we propose a novel source class distilled visual prompt that learns disentangled prompts of semantic (e.g., class) and domain (e.g., style) from a few images. Learned domain prompt is then used to synthesize images of any classes in the style of target domain. We conduct studies on various target domains with the number of images ranging from one to a few to many, and show qualitative results which show the compositional generalization of our method. Moreover, we show that our method can help improve zero-shot domain adaptation classification accuracy.

==> figure/tex/exp_synthesis.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_real_id.png}
        \caption{\textsc{Real}}
        \label{fig:synthesis_real_id}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_clipart_id.png}
        \caption{\textsc{Clipart} (ID)}
        \label{fig:synthesis_clipart_id}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_infograph_id.png}
        \caption{\textsc{Infograph} (ID)}
        \label{fig:synthesis_infograph_id}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_painting_id.png}
        \caption{\textsc{Painting} (ID)}
        \label{fig:synthesis_painting_id}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_quickdraw_id.png}
        \caption{\textsc{Quickdraw} (ID)}
        \label{fig:synthesis_quickdraw_id}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_sketch_id.png}
        \caption{\textsc{Sketch} (ID)}
        \label{fig:synthesis_sketch_id}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_real_ood.png}
        \caption{\textsc{Real}}
        \label{fig:synthesis_real_ood}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_clipart_ood.png}
        \caption{\textsc{Clipart} (OOD)}
        \label{fig:synthesis_clipart_ood}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_infograph_ood.png}
        \caption{\textsc{Infograph} (OOD)}
        \label{fig:synthesis_infograph_ood}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_painting_ood.png}
        \caption{\textsc{Painting} (OOD)}
        \label{fig:synthesis_painting_ood}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_quickdraw_ood.png}
        \caption{\textsc{Quickdraw} (OOD)}
        \label{fig:synthesis_quickdraw_ood}
    \end{subfigure}
    \begin{subfigure}[b]{0.16\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figure/result/domainnet_sketch_ood.png}
        \caption{\textsc{Sketch} (OOD)}
        \label{fig:synthesis_sketch_ood}
    \end{subfigure}
    \caption{Caption}
    \label{fig:synthesis}
\end{figure*}

==> figure/tex/method_zeroshot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/alg/method_zeroshot.pdf}
    \caption{Illustration of generative zero-shot transfer. Source-class agnostic (SCA) prompt is tuned on the target in-domain distribution (\eg, sketch images of goldfish and chihuahua). By combining class tokens of the source model and SCA prompt, we generate sketch images of unseen classes (\eg, volcano, palace, trolley).}
    \label{fig:method_zeroshot}
\end{figure}

==> section/_old_1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

%[[Opening statement on generative models.]]

Much progress has been made for conditional generative models, from class-conditional models based on generative adversarial networks~\cite{goodfellow2014generative,brock2018large}, diffusion models~\cite{dhariwal2021diffusion} or generative vision transformers~\cite{esser2021taming,chang2022maskgit,wu2022nuwa,lezama2022improved}, to text-conditional models for image synthesis, also known as a text-to-image, DALL$\cdot$E~\cite{ramesh2021zero}, DALL$\cdot$E 2~\cite{ramesh2022hierarchical}, GLIDE~\cite{nichol2021glide}, Latent Diffusion Model~\cite{rombach2022high}, Imagen~\cite{saharia2022photorealistic} or Parti~\cite{yu2022scaling}.
%
These methods have shown an incredible power of compositional generalization for image synthesis, \eg, a famous avocado armchair image created by DALL$\cdot$E.\footnote{\url{https://openai.com/blog/dall-e/}}
%
This is believed possible in part due to the large amount of training data, often more than hundreds of millions, with the rich supervision in the form of text. However, in many practical scenarios, we may not have such a scale of data nor supervision to train generative models for the domain and task of interest.

% [[Research question]]
Here, we raise the following questions: Is the large scale training data with rich text supervision necessary for compositional generalization? Where does the ability for compositional generalization come from? In this paper, we answer these questions in part that the compositional generalization of generative models is still possible without such a large scale data and text supervision. Specifically, we show how to learn to compose semantic concepts (\eg, class) and the domain (\eg, style) using publicly available dataset with class labels (\eg, ImageNet~\cite{deng2009imagenet}) and just a few images (\eg, as low as 1) characterizing properties of the target domain. \cref{fig:teaser} showcases synthesized images by composing semantic concepts from the class-conditional generative model~\cite{chang2022maskgit} and style learned from a few images in each target domain.


% [[Our method]]
Formally, we study a task of \emph{zero-shot domain adaptive image synthesis ({\expset})}, which aims to synthesize images of novel classes belonging to the target distribution using a few training images in the target domain, as in \cref{fig:teaser}. As solving {\expset} requires disentanglement of domain and semantic knowledge, the successful demonstration of {\expset} should lead to a better understanding of compositional generalization.
%
Note that this is in contrast with the task of generative transfer learning (GTL)~\cite{wang2020minegan,shahbazi2021efficient,ojha2021few,sohn2022visual} whose goal is to synthesize images of seen classes in the target domain, where no information disentanglement required.


%
We present a simple and effective solution built on top of a state-of-the-art class-conditional transformer for image synthesis~\cite{chang2022maskgit,lezama2022improved}, which represents an image as a sequence of visual tokens, and generative visual prompt tuning~\cite{sohn2022visual} for knowledge transfer. Specifically, we present two novel components. First, source class distilled visual prompt tuning to disentangle semantic and domain information using learnable prompts of two kinds, semantic and domain. Second, domain adaptive classifier-free guidance (CFG) that extends CFG~\cite{ho2022classifier,gafni2022make,yu2022scaling} across domains to improve both visual fidelity and domain adaptability. Our method is \emph{simple}, introducing only two extra tokens to the pretrained transformer, and \emph{efficient}, introducing less than $10$k parameters trained within 10 minutes on a single GPU or TPU. Finally, as shown in \cref{sec:exp}, our method is effective.


%
%We build our method on the class-conditional MaskGIT~\cite{chang2022maskgit}, a non-autoregressive vision transformer for image synthesis by representing an image as a sequence of visual tokens.
%
%Moreover, we adopt generative visual prompt tuning~\cite{sohn2022visual} that prepends learnable prompts to visual token sequence to adapt to the target domain. Specifically, we propose a novel source class distilled visual prompt tuning that makes use of domain and semantic prompts to disentangle domain and class information, respectively. 


% [[Experiment]]
We assess the success of our method in three ways. First, we conduct a qualitative study when only a few images are available from various target domains for training by visualizing synthesized images. We ablate design choices of our method to provide insights into how it works. Second, we report quantitative metrics on a newly proposed benchmark based on an ImageNet-R~\cite{hendrycks2021many}, which comes with many visual domains and their labels. Third, we make use of generated images by our method to solve zero-shot domain adaptation~\cite{peng2018zero,jhoo2021collaborative} on the Office-home dataset~\cite{venkateswara2017deep}. Experimental results show our method is able to synthesize images of unseen classes in the target domain, indicating a compositional generalization of semantic and domain information.




\iffalse
Generative transfer learning (GTL)~\cite{wang2020minegan,shahbazi2021efficient,ojha2021few,sohn2022visual} offers an efficient way of learning generative models from small amounts of data available from the target domain by transferring knowledge from the powerful source models trained on a large-scale labeled data. Despite their practical value, GTL has not been widely studied compared to the transfer learning~\cite{kolesnikov2020big} and domain adaptation~\cite{csurka2017comprehensive} for discriminative tasks (\eg, classification). While some existing works based on GANs~\cite{wang2020minegan,mo2020freeze,shahbazi2021efficient,ojha2021few} and generative vision transformers~\cite{sohn2022visual} have shown a promise, their generation capabilities are limited by the training data in the target domain. Importantly, these methods do not offer a way to synthesize by composing rich semantic knowledge (\eg, class) in the source model and target domain information.

%
In this work, we introduce a new task, \emph{zero-shot domain adaptive image synthesis} (ZDAIS), that studies knowledge transfer and composition of conditional generative models.
%
For example, given reference images of \emph{Van Gogh painting} of ``house'', we aim to synthesize \emph{Van Gogh painting} of ``chihuahua'', ``volcano'', ``convertible'' and so on, as illustrated in \cref{fig:teaser}.
%
As mentioned, previous works are capable of synthesizing \emph{Van Gogh painting} style images of ``house'' from a few training data~\cite{ojha2021few,sohn2022visual}, but their models cannot generate any other images but house. We emphasize \emph{zero-shot} as we look for generating images of unseen classes in the target domain. Note that our task definition is consistent with zero-shot domain adaptation~\cite{peng2018zero,jhoo2021collaborative}, but we tackle an image synthesis task instead of classification.

There are two key challenges -- how to learn a domain information from a few training images, and how to compose learned domain information with existing class information of the source model.
%
In this paper, we tackle with a class-conditional MaskGIT~\cite{chang2022maskgit}, a non-autoregressive vision transformer for image synthesis, for two reasons. First, it achieves a strong performance on class-conditional image synthesis. Second, thanks to the transformer~\cite{vaswani2017attention,dosovitskiy2020image}, learning and adapting to a new domain and task could be made efficient with the visual prompt tuning~\cite{jia2022visual,sohn2022visual}. 


Moreover, we present two novel components for {\expset}. First, we propose a source class distilled visual prompt tuning. Two types 


that learns to disentangle domain and semantic information from a few training images. This is done by prepending both source 
%



To learn a domain information, we propose

Our method is efficient -- it only introduces less than $10$k parameters and could be trained within 10 minutes on a single GPU or TPU.

Our method is effective, as shown in experiments.

In addition, our method is generic and may work as well for other transformer-based conditional generative models~\cite{wu2022nuwa,gafni2022make,yu2022scaling,villegas2022phenaki}.

We conduct an extensive study for {\expset}. We first conduct a qualitative study when there are only a few (\eg, as low as 1) number of training images from various target domains. We ablate design choices of our method to provide insights on how it works. Then, since there is no established benchmark for quantitative study, we propose a new benchmark using an ImageNet-R~\cite{hendrycks2021many} that comes with many visual domains and their labels. Our method achieves lower FIDs than baselines, suggesting that it synthesizes images of novel classes in the target domain better.
%
Finally, we also demonstrate the usefulness of {\expset} in zero-shot domain adaptation~\cite{jhoo2021collaborative}, where synthetic images of novel classes are used to train a classifier of the target domain.
\fi



\iffalse
In this work, we study transfer learning methods for generative vision transformers. Among several alternatives, we are interested in investigating prompt~\cite{lester2021power} and prefix~\cite{li2021prefix} tuning methods for generative visual transfer learning, as they are shown to be effective and parameter efficient in adopting large language models to the downstream tasks, as well as some discriminative tasks in computer vision~\cite{jia2022visual}. 

%
For generative visual prompt tuning, there are a few important design choices when building prompt token generators. \textbf{First}, different from discriminative models, the generative model may be conditioned on various condition variables, such as a class, attribute or instance, for controllable generation. As such, prompt token generator should be susceptible to condition variables. \textbf{Second}, having a compact representation of a condition variable is desirable for downstream applications of generative models, such as an image editing and manipulation. \textbf{Optionally}, they should be able to distill class-specific knowledge of the source data. Source class knowledge could be used to disentangle visual object concepts and the style of the target data distribution and allows zero-shot transfer for image synthesis.


%
To this end, we propose a prompt token generator that generates a set of learnable tokens, where a subset of them are used to distill class-specific knowledge of source data. 
\fi


%\lu{The format of Fig.1 looks too similar to the other paper. Consider changing it?}

==> setup/math.tex <==
\usepackage{amsmath,amsfonts,bm}

\def\argmax{\mathop{\rm argmax}}%
\def\argmin{\mathop{\rm argmin}}%


\def\bx{\bm{x}} %
\def\bxp{\bm{x}^{\prime}} %
\def\bxpp{\bm{x}^{\prime\prime}} %
\def\tbx{\tilde{\bm{x}}} %
\def\hbx{\hat{\bm{x}}} %
\def\ex{e(\bm{x})}
\def\tex{e({\tilde{\bm{x}}})}

\def\by{\bm{y}} %
\def\byp{\bm{y}^{\prime}} %
\def\bypp{\bm{y}^{\prime\prime}} %
\def\tby{\tilde{\bm{y}}} %
\def\ty{\tilde{{y}}} %
\def\hby{\hat{\bm{y}}} %
\def\ey{e(\bm{y})}
\def\tey{e({\tilde{\bm{y}}})}

\def\vw{\bm{w}}


\def\anchor{\overline{D}}

\def\reg{R_{\mathrm{LC}}}


\def\bv{\bm{v}} %
\def\tv{\tilde{v}} %
\def\tbv{\tilde{\bm{v}}} %

\usepackage{amsmath,amsfonts}
\usepackage{bbm}

\newcommand{\eat}[1]{} % ignores argument


%GAN
\def\pd{p_d(\bx)} %
\def\pg{p_g(\bx)} %
\def\pz{p_z(\bx)} %
\def\Dx{D(\bx)} %
\def\Dsx{D^*(\bx)} %



\def\N{\mathcal{N}} %
\def\Z{\mathcal{Z}} %
\def\E{\mathop{\mathbb{E}}} %

==> table/main_synthesis.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
        Source & \multicolumn{5}{c|}{DomainNet \textsc{real}} & \multicolumn{2}{c}{ImageNet} \\ \midrule
        Target & \textsc{Clipart} & \textsc{Infograph} & \textsc{Painting} & \textsc{Quickdraw}  & \textsc{Sketch} & \textsc{Sketch} & \textsc{Sketch}$^{\dagger}$ \\
        \midrule
        O2TO ($\downarrow$) & 19.4{\footnotesize$\pm1.4$} & 16.5{\footnotesize$\pm1.4$} & 18.8{\footnotesize$\pm1.1$} & 28.6{\footnotesize$\pm2.6$} & 20.1{\footnotesize$\pm1.9$} & & 14.8{\footnotesize$\pm0.6$} \\
        I2TI ($\downarrow$) & 21.4{\footnotesize$\pm2.6$} & 19.2{\footnotesize$\pm1.6$} & 16.8{\footnotesize$\pm1.8$} & 20.2{\footnotesize$\pm1.3$} & 19.7{\footnotesize$\pm1.7$} & -- & 16.2{\footnotesize$\pm0.5$} \\
        O2TI ($\uparrow$) & 40.2{\footnotesize$\pm4.1$} & 23.1{\footnotesize$\pm1.9$} & 47.0{\footnotesize$\pm5.7$} & 21.6{\footnotesize$\pm1.1$} & 35.4{\footnotesize$\pm3.4$} & -- & 41.8{\footnotesize$\pm3.4$} \\
        O2SO ($\uparrow$) & 65.7{\footnotesize$\pm2.7$} & 96.8{\footnotesize$\pm4.2$} & 36.7{\footnotesize$\pm1.6$} & 279.0{\footnotesize$\pm4.5$} & 77.7{\footnotesize$\pm4.5$} &  & 81.0{\footnotesize$\pm0.8$} \\
        \midrule
        Supervised & \\
    \bottomrule
    \end{tabular}
    \caption{Zero-shot image synthesis on DomainNet and ImageNet. FID scores averaged over 5 folds (\eg, super-classes) and their standard errors are reported. Datasets covering natural images (DomainNet \textsc{real}, ImageNet) are used as source domains, and those with different styles are used as target domains. Various FID scores are reported based on the generation (\eg, target \textbf{I}n- or \textbf{O}ut-of-distribution) and the reference (\eg, \textbf{S}ource or \textbf{T}arget). We provide FID scores for models trained on the entire target data (supervised) as FID lower bounds.}
    \label{tab:main_zeroshot_synthesis}
\end{table*}

==> table/num_params.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l|c|c|c}
    \toprule
     &  $L\,{=}\,1$ & Fact. over $L$ & None \\
    \midrule
        $S\,{=}\,1$ & 0.08 & 0.10 & 1.84 \\
        Fact. over $S$ & 0.13 & 0.14 & 3.02 \\
        None & 4.92 & 6.09 & 117.96 \\
    \bottomrule
    \end{tabular}
    \caption{Number of learnable parameters in millions for different factorizations of the class-conditional prompt token generator. We use the prompt length $S\,{=}\,64$, the number of transformer layer $L\,{=}\,24$, the number of class $C\,{=}\,100$, and the token dimension $D\,{=}\,768$. $\dagger$ refers to a factorization over sequence dimension.}
    \label{tab:num_params_for_prompt}
\end{table}

==> table/problem_comparison.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.7\linewidth}{!}{%
    \begin{tabular}{c|c|c}
    \toprule
         & GTL~\cite{shahbazi2021efficient,sohn2022visual} & ZDAIS (ours) \\
         \midrule
        Train & \multicolumn{2}{c}{$(\mathcal{X}_{\mathrm{src}}, \mathcal{Y}_{\mathrm{src}})$, $(\mathcal{X}_{\mathrm{tgt}}, \mathcal{Y}_{\mathrm{tgt}})$} \\ \midrule
        Synthesis & $(\mathcal{X}_{\mathrm{tgt}}, \mathcal{Y}_{\mathrm{tgt}})$ & $(\mathcal{X}_{\mathrm{tgt}}, \mathcal{Y}_{\mathrm{src}}\backslash\mathcal{Y}_{\mathrm{tgt}})$\\
    \bottomrule
    \end{tabular}
    }
    \vspace{0.05in}
    \caption{Comparison of generative transfer learning (GTL) and zero-shot domain adaptive image synthesis (ZDAIS). %ZDAIS aims to synthesize images of a class not only in the target, but also in the source domain, which may contain significantly more classes. %\luisa{Should we change $(\mathcal{Y}{\mathrm{src}}\cup\mathcal{Y}{\mathrm{tgt}})$ with $(\mathcal{Y}_{\mathrm{src}}\backslash \mathcal{Y}_{\mathrm{tgt}})$ to make it more consistent with the body text (Lines 261-263 from Sec. 4.1)?}
    }
    \label{tab:learning_setting_comparison}
    \vspace{-0.2in}
\end{table}

